The xx205 System for the VoxCeleb Speaker Recognition Challenge 2020

This report describes the systems submitted to the first and second tracks of the VoxCeleb Speaker Recognition Challenge (VoxSRC) 2020, which ranked second in both tracks. Three key points of the system pipeline are explored: (1) investigating multiple CNN architectures including ResNet, Res2Net and dual path network (DPN) to extract the x-vectors, (2) using a composite angular margin softmax loss to train the speaker models, and (3) applying score normalization and system fusion to boost the performance. Measured on the VoxSRC-20 Eval set, the best submitted systems achieve an EER of $3.808\%$ and a MinDCF of $0.1958$ in the close-condition track 1, and an EER of $3.798\%$ and a MinDCF of $0.1942$ in the open-condition track 2, respectively.

==> input_representation.tex <==
\begin{table}[h]
 \renewcommand\thetable{1}
 \caption{Hyper-parameters for input representation.}
  \centering
  \label{table:input}
  \begin{tabular}{r l }
  
  %\Xhline{2\arrayrulewidth}
  \toprule

   Hyper-parameter &  \\
  \hline
  frame length & 25ms\\
  
  shift size & 10ms \\
  
  number of FFT bins & 512\\
  
  number of filters & 64\\
  
  pre-emphasis & with 0.97 coefficient \\
  
  normalization & mean \& variance normalization\\
   \bottomrule
  \end{tabular}
\end{table}

==> results.tex <==
\begin{table*}[h]
\caption{Results on the VoxCeleb and VoxSRC test sets.
The figures in bold represent the best results for each metric, excluding the fusion outputs.
{\bf AP:} Angular Prototypical.
{\bf BN:} Batch Normalisation on the speaker embeddings.
$\dag$ This method uses score normalisation as a post-processing step.}
\label{table:results}
\footnotesize
\setlength{\tabcolsep}{4pt}
\renewcommand\arraystretch{1.2}
\centering
\begin{tabular}{ l l l l | r  r | r r | r r | r r | r r  }
\toprule
 \textbf{Config.} & \textbf{Loss} & \textbf{Aug.} & \textbf{BN}   & \multicolumn{2} {c|} {\bf VoxCeleb1}& \multicolumn{2} {c|} {\bf VoxCeleb1-E cl.} & \multicolumn{2} {c|} {\bf VoxCeleb1-H cl.} & \multicolumn{2} {c|} {\bf VoxSRC 2019} & \multicolumn{2} {c} {\bf VoxSRC 2020 Val} \\
    &     &   & & \textbf{EER} & \textbf{MinDCF} & \textbf{EER} & \textbf{MinDCF}  & \textbf{EER} & \textbf{MinDCF}  & \textbf{EER} & \textbf{MinDCF} & \textbf{EER} & \textbf{MinDCF} \\ 
\midrule

FR-34~\cite{chung2020defence} & AP           & \xmark & \xmark & 2.22 & - & - & - & - & - & - & -           & - & - \\
Sys 1~\cite{zeinali2019but} & Softmax~$\dag$ & \cmark & \xmark & - & - & 1.35 & - & 2.48 & - & - & -        & - & - \\
Fusion~\cite{zeinali2019but} & - & - & - & - & - & 1.14 & - & 2.21 & - & 1.42 & -        & - & - \\
% Sys A4~\cite{garcia2020jhu} & AM-Softmax & \cmark & \xmark & - & - & 1.61 & - & - & - & 1.91 & -        & - & - \\
Sys A5~\cite{garcia2020jhu} & AM-Softmax & \cmark & \xmark & - & - & 1.51 & - & - & - & 1.72 & -        & - & - \\
Fusion~\cite{garcia2020jhu} & - & - & - & - & - & 1.22 & - & - & - & 1.54 & -        & - & - 
\\ \midrule

Q / SAP & AM-Softmax & \xmark & \cmark &  2.20  & 0.139 &          2.10 & 0.137 &     3.67 & 0.213  &    2.31 & 0.144         & 5.43 & 0.295  \\
Q / SAP & AAM-Softmax & \xmark & \cmark &  2.13 & 0.138 &          2.12 & 0.140 &     3.52 & 0.211  &    2.33 & 0.145         & 5.19 & 0.290  \\
Q / SAP & AP          & \xmark & \cmark &  1.90 & 0.133 &          1.99 & 0.144 &     3.80 & 0.243  &    2.24 & 0.152         & 5.67 & 0.325 \\
Q / SAP & AP+Softmax & \xmark & \cmark &  1.85  & 0.119 &          1.96 & 0.138 &     3.65 & 0.233  &    2.16 & 0.146         & 5.49 & 0.311  \\ \midrule

H / ASP & AM-Softmax & \cmark & \xmark &  1.64  & 0.115 &       1.67 & 0.114 &     3.07 & 0.191  &     1.88 & 0.112          & 4.59 & 0.263 \\
H / ASP & AAM-Softmax & \cmark & \xmark &  1.59  & 0.113 &       1.50 & 0.105 &    2.91 & 0.181  &    1.74 & 0.103          & 4.40 & 0.244  \\
H / ASP & AP          & \cmark & \xmark & 1.50  & 0.126 &       1.69 & 0.120 &     3.39 & 0.217  &    1.92 & 0.128          & 5.09 & 0.288 \\
H / ASP & AP+Softmax  & \cmark & \xmark &  {\bf 1.18}  & {\bf 0.086} &      {\bf 1.21} & {\bf 0.086} &     {\bf 2.38} & {\bf 0.154}  &     {\bf 1.46} & {\bf 0.088}         & {\bf 3.79} & {\bf 0.213} \\ \midrule

H / ASP & AM-Softmax & \cmark & \cmark &  1.49  & 0.104 &       1.45 & 0.099 &     2.64 & 0.165  &     1.64 & 0.097         & 4.05 & 0.231  \\
H / ASP & AAM-Softmax & \cmark & \cmark &  1.28  & {\bf 0.086} &      1.34 & 0.091 &     2.48 & 0.155  &    1.61 & 0.093          & 3.81 & 0.218 \\
H / ASP & AP          & \cmark & \cmark & 1.43  & 0.113 &       1.45 & 0.105 &     2.91 & 0.189  &    1.74 & 0.117          & 4.43 & 0.262 \\
H / ASP & AP+Softmax  & \cmark & \cmark &  1.25  & 0.087 &      1.34 & 0.095 &     2.71 & 0.175  &     1.49 & 0.102         & 4.24 & 0.243  \\
 \bottomrule
\end{tabular} 
\end{table*}
